Data Quality in Crowdsourcing and Spamming Behavior Detection

As crowdsourcing emerges as an efficient and cost-effective method for obtaining labels for machine learning datasets, it is important to assess the quality of crowd-provided data, so as to improve analysis performance and reduce biases in subsequent machine learning tasks. Given the lack of ground truth in most cases of crowdsourcing, we refer to data quality as annotators' consistency and credibility. Unlike the simple scenarios where Kappa coefficient and intraclass correlation coefficient usually can apply, online crowdsourcing requires dealing with more complex situations. We introduce a systematic method for evaluating data quality and detecting spamming threats via variance decomposition, and we classify spammers into three categories based on their different behavioral patterns. A spammer index is proposed to assess entire data consistency, and two metrics are developed to measure crowd workers' credibility by utilizing the Markov chain and generalized random effects models. Furthermore, we showcase the practicality of our techniques and their advantages by applying them on a face verification task with both simulation and real-world data collected from two crowdsourcing platforms.

==> sections/1abstract.tex <==
\csname documentclass\endcsname[../main.tex]{subfiles}
\begin{document}
As crowdsourcing emerges as an efficient and cost-effective method for obtaining labels for machine learning datasets, it is important to assess the quality and reliability of crowd-provided data, so as to improve the performance and reduce the bias of machine learning models. Since crowdsourcing aims to gain ground truth for most cases, we refer data reliability to annotators' consistency and outline the variance related to annotators as the indicator of how they are self-consistent. Unlike the simple scenarios where Kappa coefficient and intraclass correlation coefficient usually can apply, online crowdsourcing requires dealing with more complex situations (e.g. multiple annotations for single tasks and categorical responses). We present a systematic method to evaluate data quality and detect crowdsourcing spammers (classifying spammers into three categories based on their different behavioral types) via the Markov chain and generalized random effects models and show how data quality is associated with the amount of spamming behavior and accuracy. We also demonstrated the usability of our methods in a face verification task via both simulation and real-world data collected from two representative crowdsourcing platforms, as well as providing empirical procedures for assessing data quality and identifying potential spamming behaviors.  


\end{document}
